Decentralized Multi-Agent Actor-Critic with Generative Inference

Recent multi-agent actor-critic methods have utilized centralized training with decentralized execution to address the non-stationarity of co-adapting agents. This training paradigm constrains learning to the centralized phase such that only pre-learned policies may be used during the decentralized phase, which performs poorly when agent communications are delayed, noisy, or disrupted. In this work, we propose a new system that can gracefully handle partially-observable information due to communication disruptions during decentralized execution. Our approach augments the multi-agent actor-critic method's centralized training phase with generative modeling so that agents may infer other agents' observations when provided with locally available context. Our method is evaluated on three tasks that require agents to combine local and remote observations communicated by other agents. We evaluate our approach by introducing both partial observability during decentralized execution, and show that decentralized training on inferred observations performs as well or better than existing actor-critic methods.

==> settings/kcorder_includes.tex <==
\usepackage{amsmath, amsfonts, amsthm}
\usepackage{mathtools}
\usepackage{graphicx}
\usepackage{blindtext}
\usepackage[at]{easylist}
\usepackage{todonotes}
\usepackage{algorithm}
\usepackage{tabu}
\usepackage{booktabs}
\usepackage{geometry}

\usepackage[pdfencoding=auto,psdextra]{hyperref}
\usepackage{cleveref, hypcap}

\usepackage[noend]{algpseudocode}

\usepackage{import}
\usepackage[shortlabels,inline]{enumitem} % for more enumeration options
\usepackage{xspace}
\usepackage{subcaption}
\usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox
\usepackage{marginnote}
% \usepackage{titling}

\usepackage{xcolor} % for more colors
\usepackage{soul} % provides \hl{text to be highlighted}

% \usepackage{ifthen}
% \usepackage{xparse}



% command for creating easier math macros to be placed in text
% \anycmd{\myvar}{var},  equivalent to:
% -> \newcommand{\myvar}{\any{var}}
% Now I can use the variable \myvar more easily! Still need the math mode for writing its square $\myvar^2$.
\newcommand{\any}[1]{\ensuremath{{#1}}\xspace}
\newcommand{\anycmd}[2]{\newcommand{#1}{\any{#2}}}

% supposed to have an optional argument for g, not working correctly..
% \DeclareDocumentCommand \anyfn { m g }{%
%     \IfNoValueTF {#2} {\any{#1}} {\any{#1(#2)}}%
% }
% EXAMPLE OF CORRECT USAGE:
% \DeclareDocumentCommand\sec{ m g }{%
%     {#1%
%         \IfNoValueF {#2} { and #2}%
%     }%
% }
% (\sec{Hello})
% (\sec{Hello}{Hi})


%% COLOR / EDITING %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% set these to not break when using soul's \hl below!
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7

\newcommand{\hlc}[2][yellow]{ {\sethlcolor{#1} \hl{#2}} }

% possibly remove, reword, or verify accuracy of highlighted text
\newcommand{\remove}[1]{\hlc[red]{#1}}
\newcommand{\reword}[1]{\hlc[cyan]{#1}}
\newcommand{\verify}[1]{\hlc[green]{#1}}
\newcommand{\addabove}[1]{\hlc[pink]{#1}}


% these are shortcuts for coloring text a set color, which are purple or teal here. Note: using \purple for comments, and \teal for research-specific comments/questions.
% Ex: \purple{hey, here's some text oh jeez...
%				newlines are okay too!}
\newcommand{\purple}[1]{{\color{purple}#1}} % needs revision
\newcommand{\teal}[1]{{\color{teal}#1}}		% note/question to self

% need to fill in something with \blank space
\newcommand{\blank}{\underline{\ \ \ \ \ \ \ }}
% syntax: \ignore{x} - does an inline comment, so x is ignored by LaTeX
\newcommand{\ignore}[1]{}

% \TODO is a shortcut for inline todo items from the todonotes package. Makes a bubbled comment with default color, which is added to the To Do List at top of document if \listoftodos is called on the title page.
% Can specify different html-named color with an option, like: \TODO[cyan]{hello world}
% (the \color{black} is to avoid other colored text in colored bubbles)
\newcommand{\TODO}[2][orange]{\todo[inline,color=#1]{\color{black}#2}}
\newcommand{\selfnote}[1]{\TODO[cyan]{#1}}

% syntax: \margindef{x}
% will write 'x' in the margin (left margin if \reversemarginpar is set below) and will make 'x' boldface inline 
\newcommand{\margindef}[1]{\textbf{#1}\marginnote{\MakeUppercase{#1}}}
\reversemarginpar % sets the margin note to the left side 
\renewcommand*{\marginfont}{\tiny} % probably one of {\tiny, \scriptsize, \footnotesize} 

%%%% MATH  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% these are from the amsthm package, and I have defined:
%   thmN: writes a Theorem with a numbering. May want to re-define to specify the option for the sectioning level for numberings.
% 	defnN: writes a Definition with a numbering, based on the thmN numbering
%	thm: Theorem with no number
%	defn: Definition with no number
\theoremstyle{plain}    % boldface heading, italicized body
\newtheorem{thmN}{Theorem}
\newtheorem*{thm}{Theorem}
\newtheorem{propN}[thmN]{Proposition}
\newtheorem*{prop}{Proposition}
\newtheorem{corollaryN}[thmN]{Corollary}
\newtheorem*{corollary}{Corollary}
\newtheorem{lemmaN}[thmN]{Lemma}
\newtheorem*{lemma}{Lemma}

\theoremstyle{definition}   % boldface heading, normal body
\newtheorem{defnN}{Definition}
\newtheorem*{defn}{Definition}
\newtheorem{exampleN}{Example} % doesn't follow thmN numbering
\newtheorem*{example}{Example}

% shortcut for using aligned equations, but can be used inline
% syntax: \eq{x^2 &= y + z\\y &= \sqrt[3]{z}}   %(1)   multi-line
%		  \eq{x^2+y^2 &= 1  &  z^3 &=sqrt[5]{x}} %(2) 	multi-column
\newcommand{\eq}[1]{\begin{equation*}\begin{aligned}#1\end{aligned}\end{equation*}}
% this shortcut will number the equation
\newcommand{\eqn}[1]{\begin{equation}\begin{aligned}#1\end{aligned}\end{equation}}

% syntax: \overbar{x}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

% for vector variables
\newcommand{\vect}[1]{\textbf{#1}}

% \parens{wrap text in parentheses}
% can use option for size, e.g. \parens[\Big]{text}
\DeclarePairedDelimiter{\parens}{\lparen}{\rparen}
% \braces{dog} -->  {dog}
\DeclarePairedDelimiter{\braces}{\lbrace}{\rbrace}
% \bracks{dog} -->  [dog]
\DeclarePairedDelimiter{\bracks}{\lbrack}{\rbrack}

% Declaring argmin and argmax for math mode.
% Ex:
%	$\argmin x : x^2 < 410y^{10.5}$
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% Blackboard E for expectation 
\DeclareMathOperator{\expect}{\mathbb{E}}




% lists %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% shortcuts for lists (mostly for embedding)
\newcommand{\enumlist}[1]{\begin{enumerate}#1\end{enumerate}}
\newcommand{\itemlist}[1]{\begin{itemize}#1\end{itemize}}




% reference commands/options  %%%%%%%%%%%%%%%%%%%%%%%%

% \anchorref{} takes a figure label and will do better referencing, including hyperref with the cleveref modification to not miss the floating element when pdf jumps to location since captions are most commonly below the image and inserts the type of reference for you.
% Ex: \anchorref{payoffs} ->
\newcommand\anchorref[1]{\hyperref[#1]{\cref{#1}}}
\newcommand\Anchorref[1]{\hyperref[#1]{\Cref{#1}}} % capitalized

% \anchoralg is a label for algorithms. See \anchorref
\newcommand\anchoralg[1]{\hyperref[#1]{algorithm \ref{#1}}}
\newcommand\Anchoralg[1]{\hyperref[#1]{Algorithm \ref{#1}}} % capitalized

% doesn't work for links with special characters... 
\newcommand{\linktext}[2]{\href{#1}{\color{blue}{#2}}}

%% hypersetup needed when using hyperref!
\newcommand{\setpdfinfo}[2]{\hypersetup{pdfinfo={
Title={#1},
Author={#2}
}}}




% Other options: %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% graphicx alters page size a little..
% this is for consistency
% \setlength{\pdfpagewidth}{8.5in}
% \setlength{\pdfpageheight}{11in}

% margin settings for page 
% \geometry{margin=1in} 


% file location settings  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\graphicspath{{graphics/}}


==> settings/kcorder_recipes.tex <==
% This file shouldn't be called! The LaTeX code here is only 
% meant to be copied as a template later use. 

% figures %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\includegraphics[width=\linewidth]{approxVisualExplanation}
\caption{Blah}
\label{fig:blah}
\end{figure}


% tables %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\label{table:blah}
% Example notation table is 0.9*\textwidth with two columns: 
% 	first is right-aligned (r) and second is left-aligned
% 	and takes up all remaining space (X[l])
\begin{tabu} to 0.9\textwidth { | r | X[l] | }
	\hline
	\multicolumn{2}{|c|}{\textbf{Notation}} \\ \hline
%     symbol   &  definition  \\ \hline 
\end{tabu}
\caption{Blah}
\end{table}


% WRITING %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
% Many abstracts follow a five-element organization:
% 1. A general statement introducing the broad research area of the particular topic being investigated.
% 2. An explanation of the specific problem (difficulty, obstacle, challenge) to be solved.
% 3. A review of existing or standard solutions to this problem and their limitations.
% 4. An outline of the proposed new solution.
% 5. A summary of how the solution was evaluated and what the outcomes of the
% evaluation were.
\end{abstract}

